Overcoming the Long Horizon Barrier for Sample-Efficient Reinforcement Learning with Latent Low-Rank Structure

The practicality of reinforcement learning algorithms has been limited due to poor scaling with respect to the problem size, as the sample complexity of learning an $\epsilon$-optimal policy is $\tilde{\Omega}\left(|S||A|H^3 / \epsilon^2\right)$ over worst case instances of an MDP with state space $S$, action space $A$, and horizon $H$. We consider a class of MDPs for which the associated optimal $Q^*$ function is low rank, where the latent features are unknown. While one would hope to achieve linear sample complexity in $|S|$ and $|A|$ due to the low rank structure, we show that without imposing further assumptions beyond low rank of $Q^*$, if one is constrained to estimate the $Q$ function using only observations from a subset of entries, there is a worst case instance in which one must incur a sample complexity exponential in the horizon $H$ to learn a near optimal policy. We subsequently show that under stronger low rank structural assumptions, given access to a generative model, Low Rank Monte Carlo Policy Iteration (LR-MCPI) and Low Rank Empirical Value Iteration (LR-EVI) achieve the desired sample complexity of $\tilde{O}\left((|S|+|A|)\mathrm{poly}(d,H)/\epsilon^2\right)$ for a rank $d$ setting, which is minimax optimal with respect to the scaling of $|S|, |A|$, and $\epsilon$. In contrast to literature on linear and low-rank MDPs, we do not require a known feature mapping, our algorithm is computationally simple, and our results hold for long time horizons. Our results provide insights on the minimal low-rank structural assumptions required on the MDP with respect to the transition kernel versus the optimal action-value function.

==> sigmetrics/main_text/discussion.tex <==
\subsection{Discussion}\label{sec:disc}
We next discuss the suboptimality of our sample complexity bounds with respect to the horizon, rank, and incoherence parameter. 

\paragraph{Optimal dependence on $H$.} To better understand, what is optimal with respect to $H$, we next present a simple lower bound in our setting. We can easily establish a $d(|S|+|A|)H^3/\eps^2$ lower bound from lower bounds provided in literature; existing lower bounds from \cite{sidford2019nearoptimal} prove the necessity of $d|S|H^3/\eps^2$ samples for a homogeneous MDP with $|S|$ states and $d$ actions. Replicating each action $|A|/d$ times results in a rank-$d$ MDP with $|A|$ actions that is at least as hard as the original MDP. In contrast, existing lower bounds for linearly-realizable MDPs \cite{wang2021exponential, weisz2021exponential} are not applicable in our setting because they show that $\exp(\min(d, H))$ samples are needed but construct an MDP with $|A| = 2^d$. Hence, this lower bound is linear in $|A|$, which is no stronger than the above simple linear lower bound. \cycomment{Rewrite this paragraph clearer.}

The above simple lower bound shows that an $H^3$ dependence in the homogeneous low-rank MDP setting is required which is similar to our $H^5$ dependence from LR-EVI under incoherence and low Tucker rank transition kernels in the \emph{non-homogeneous} low-rank MDP setting. To further decrease the dependence on $H$, we would need to use techniques like the Total Variance technique in \cite{sidford2019nearoptimal}; however, it requires estimating the variance of each $\hat{Q}(s,a)$. While one can show that the variance of the Bellman operator is low rank under our strongest assumption, it has rank $O(d^2)$. Hence, attempts to achieve the optimal dependence on $H$ while using low-rank methods will incur a significantly worse dependence on $d$, i.e., $d^{10}$.  

\paragraph{Optimal dependence on $d$.} While any algorithm must at least incur linear dependence on the rank $d$, an optimal dependence on $d$ would require significant innovation in the matrix estimation literature, as all current entrywise error guarantees suboptimal with respect to $d$ \cite{serl, abbe2020entrywise, chen2019noisy}. 

\paragraph{Optimal dependence on $\mu$.} To show that the sample complexity must incur some dependence on $\mu$, we present the following lemma. 
\begin{lemma}\label{lem:incoLB}
There exists a low-rank $d$, $\mu$-incoherent MDP with $H=1, |S| = |A|= n$ such that $\mu^2d^2 + dn$ samples are required to recover the optimal action-value function. 
\end{lemma}
Hence, we show that there is at least an additive dependence on the incoherence parameter in the sample complexity bound. While in the classical matrix estimation literature, a multiplicative dependence on $\mu$ is shown in the sample complexity, the proofs crucially require the uniform sampling pattern. Showing a multiplicative dependence on $\mu$ is necessary with an adaptive sampling pattern is an exciting open question. On the other hand, one could create a matrix estimation method under adaptive sampling that only incurs additive dependence on $\mu$. Either of the two results would further strengthen our novel sample complexity bounds as the lower bound adds justification as to why our bounds have a multiplicative dependence on $\mu$, or we adapt the new matrix estimation method and obtain an additive dependence on $\mu$, which allows our algorithms to be sample efficient on significantly more coherent problems.



==> sigmetrics/main_text/double_exponential.tex <==
\section{Doubly Exponential Growth in Long Horizons}
\label{sec:double_exp}

\cycomment{Replace this section with Yudong's new Lower Bound + a discussion?}
While one may hope to learn the optimal action-value functions when only assuming that $Q^*_h$ is low rank, we argue that the problem is more nuanced. Specifically, we present an example where, even for the seemingly easier problem of policy evaluation, a direct combination of value iteration and low-rank matrix estimation results in an estimation error of the action-value function growing doubly exponentially with respect to $H$. 

Consider an MDP $(S, A, P, R, H)$ where $S = A = \{1,2\}$ and $Q^*_h $ is rank-1 for all $h\in[H]$, and $\pi$ is an optimal policy to be evaluated. Suppose that we are given an inexact terminal estimate $\hat{V}^\pi_H$ and recurse backward in time $h=H,H-1,\ldots,1$. For the state-action pairs $(s,a) \in \Omega:= \{ (1,1),(1,2),(2,1)\}$, we compute an estimate of $Q_h^*(s,a)$ using the exact Bellman operator given $\hat{V}^\pi_{h+1}$ according to
$
\hat{Q}^\pi_h(s,a) = r_h(s,a) + [P_h \hat{V}^\pi_{h+1}] (s,a), 
\forall (s,a) \in \Omega.
$
To estimate $Q_h^*(2,2)$ under this rank-1 setting, we solve the natural  least-squares formulation
\begin{equation}
\label{eq:least_squares}
\min_{u, v \in \R^2} \big(u_1 v_1 - \hat{Q}^\pi_h(1,1) \big)^2 + \big(u_1 v_2 - \hat{Q}^\pi_h(1,2) \big)^2 + \big(u_2 v_1 - \hat{Q}^\pi_h(2,1) \big)^2
\end{equation}
and use the optimal $(u,v)$ to form the estimate $\hat{Q}^\pi_h(2,2) := u_2 v_2$. It is easy to see that the estimate is given in closed form by 
\begin{equation}\label{eq:est}
\hat{Q}^\pi_h(2,2) = \frac{\hat{Q}^\pi_{h}(1,2)\hat{Q}^\pi_{h}(2,1)}{ \hat{Q}^\pi_{h}(1,1)}.
\end{equation}
This estimator corresponds to the unique rank-$1$ completion of $\hat{Q}^\pi_h \in \mathbb{R}^{2\times2}$ given the entries in $\Omega$, and also coincides with the estimator used in \cite{serl}. Finally, let $\hat{V}^\pi_h$ be the value function corresponding to $\hat{Q}^\pi_h$.
%
We establish the following result, whose proof is deferred to Appendix~\ref{app:proofs}.
%
\begin{lemma}[Doubly Exponential Growth]\label{lem:de_simple}
There exists an MDP in the above setting with horizon $H$ and an optimal policy $\pi$, for which if the terminal estimate has error $ \| \hat{V}^\pi_H - V^*_H \|_\infty = \epsilon\in o(1)$, then for sufficiently large $H$, policy evaluation using the above algorithm  results in 
\[
 \| \hat{V}^\pi_1 - V^*_1 \|_\infty  = \Omega\Big((1+ \eps)^{(2^{H/2})}\Big) .
\]
\end{lemma}
In the proof, we explicitly construct an MDP and show that the estimation error $\eps_h := \| \hat{V}^\pi_h - V^*_h \|_\infty$ satisfies the recursion $ \eps_h = \eps_{h+1} + \eps_{h+1}^2$, resulting in a doubly exponential blow-up; moreover, this behavior is precisely due to the nonlinearity in the low-rank estimator~\eqref{eq:est}. A slight change to the MDP results in exponential error growth even for very small $\eps$, e.g.,  $\eps \ll 1/H$, when evaluating a near-optimal policy. This example illustrates that reinforcement learning with low-rank structure is more nuanced than its linear counterpart, and that the constant horizon assumption in~\cite{serl} is not merely an artifact of their analysis. This motivates us to consider additional assumptions, beyond $Q^*_h$ being low rank, in order to achieve stable and  sample-efficient learning with long horizons.   


%. To prove the doubly exponential growth of the initial error, we first show that the error of $\hat{V}^\pi_{h}$ follows the  recurrence relation, $\eps_h = \eps_{h+1} + \eps_{h+1}^2$, which proves that $\eps_h$ is strictly increasing as $h$ approaches one. After the error has grown to be greater than one at some time step $t$, writing out the error at time step 1, $\eps_1$, as a function of $\eps_t$ establishes the result. 


%Hence, as long as the terminal value function estimate error is non-zero, $\eps_H > 0$, and the horizon is long enough, then the error of estimating the value function of policy $\pi$ grows doubly exponentially as we recurse backwards through the horizon. 

%This example shows that without a restriction on the horizon, i.e., $H \in O(1)$, there exists MDPs in which using low-rank estimators (factored least squares and the one proposed in \cite{serl}) results in any error at the terminal step of policy evaluation growing exponentially with the horizon. Hence, additional assumptions are required to learn near-optimal policies or action-value functions in a sample-efficient manner.   

%\srscomment{Could take out the construction from this section and just give a high level comment on relating this example to the Devavrat paper.  Start off with something like, the most basic assumption in low rank MDP is stating that $Q_h^\star$ has low rank $d$.  The related work needed additional assumptions in order to get the sample complexity bound, like bounded horizon.  The following counter example highlights why this is needed, showing double exponential error propagation over the time horizon.  Highlights that using existing matrix completion techniques under assumption that only $Q_h^\star$ is low rank leads to this error.  Open question as to whether this assumption can be relaxed.  Goal of this work is using their method and understanding minimal additional assumptions we can impose, then go into that section.  That way you can get rid of the explicit construction, and even you can re-do the Lemma and just say like ``There is an MDP such that there exists some $\epsilon$ where the algorithm given in Shah has error $\Omega(e^{H})$ type of thing.''  As really the point of this lemma isn't the actual construction, but more so the exponential growth so could take out some of the detials.}

%Discussion contrasting this with when the transition kernel is low rank ....
